Disentangling data distribution for Federated Learning

Federated Learning (FL) facilitates collaborative training of a global model whose performance is boosted by private data owned by distributed clients, without compromising data privacy. Yet the wide applicability of FL is hindered by entanglement of data distributions across different clients. This paper demonstrates for the first time that by disentangling data distributions FL can in principle achieve efficiencies comparable to those of distributed systems, requiring only one round of communication. To this end, we propose a novel FedDistr algorithm, which employs stable diffusion models to decouple and recover data distributions. Empirical results on the CIFAR100 and DomainNet datasets show that FedDistr significantly enhances model utility and efficiency in both disentangled and near-disentangled scenarios while ensuring privacy, outperforming traditional federated learning methods.

==> Section/Background.tex <==
\section{Background}

\subsection{Multi-objective federated learning}

Pareto frontier...

\subsection{Attack in Federated Learning}
In this work, for our architecture, we consider all participants, including $K$ clients and the server, are \textit{honest-but-curious} adversaries. They possibly do some calculations to obtain the private data of clients by observing the model weights and updates, but they do not maliciously modify their
own inputs or parameters for the attack purpose. There are considered in our study: DLG and MI attack.\\
\textbf{DLG} Deep leakage attack is firstly proposed by \cite{zhu2020deep}, where the server tries to recover the original data based on updates and model weights. Consider $k_{th}$ client who submit its gradient $\nabla W_{pub}$ of public model. To reconstruct the raw data of client $k$, firstly initializing a dummy input $\mathbf{x}^{\prime}$ with label $\mathbf{y}^{\prime}$. Then, feeding the dummy data into the model and get the dummy gradient:

\begin{equation}
\label{dummy_grad}
\nabla W^{\prime}_{pub}=\frac{\partial \ell\left(F\left(\mathbf{x}^{\prime}, W\right), \mathbf{y}^{\prime}\right)}{\partial W}.
\end{equation}

\begin{equation}
\label{eq:dlg}
    \mathbf{x}^{\prime *}, \mathbf{y}^{\prime *}=\underset{\mathbf{x}^{\prime}, \mathbf{y}^{\prime}}{\arg \min }\left\|\nabla W_{pub}^{\prime}-\nabla W_{pub} \right\|^{2}
\end{equation}
 where $\ell$ is the classification loss, $F$ is the forward function.

By minimizing the differences between the dummy gradients and the original gradients (as shown in equation \ref{eq:dlg}), the attackers could learn a good input $\mathbf{x}^{\prime *}$ and $\mathbf{y}^{\prime *}$. In particular, DLG could easily recover the private model's output and even recover the original image if the private model is leaked, which is similar to the white-box attack.
\\\textbf{MI} However, sometimes, the attacker may not know the weights of the private model. In this case, model inversion attack (MI \cite{he2019model}) provides a strategy to reconstruct the original image. MI attack attempts to recover the original input given the private model output as the following two cases: (1) In the white-box setting, the adversary knows the private model on the participant. (2) In the black-box setting, the model parameters on the participant are unavailable for the adversary. In our setting, we mainly consider the second case. The server may conspire with the curious client to obtain other clients' data. The server provides the updated weights and gradients of the public model to reconstruct the output of the private model, and the curious client offers his own private model as the target model.

Specifically, given the private model output $O_{prt}$ and target model $F$, MI attack learns a good dummy input $\mathbf{x}^{\prime *}$ by solving the equation \ref{eq:MIA}.
\begin{equation}
\label{eq:MIA}
    \mathbf{x}^{\prime *} =\underset{\mathbf{x}^{\prime}}{\arg \min }\left\|F(\mathbf{x}^{\prime})-O_{prt}\right\|^{2}
\end{equation}

\subsection{Periodic Neurons} \label{sec:periodic neurons}
Let $\gamma = \gamma(d) >1$ be a sequence of numbers indexed by the input dimension
$d \in N$, and let $\phi: R \to [-1,1]$ be an 1-periodic function. We denote by $\mathcal{F}_\gamma^\phi$ the function class
\begin{equation}
    \mathcal{F}_\gamma^\phi = \{ f: R^d \to [-1,1] | f(x) = \phi(\gamma<w,x>), w\in S^{d-1} \} 
\end{equation}


Note that each member of the function class $\mathcal{F}_\gamma^\phi$ is fully characterized by a unit vector $w \in S^{d-1}$. We refer such function classes as periodic neurons. 

\subsection{Security Analysis of Periodic Neurons}
\subsubsection{Average-Case Decision Problems}
In the average case decision problems the statistician receives $m$ samples from either a distribution $D$ or another distribution $D_0$, and needs to decide based on the produced samples whether the generating distribution is $D$ or $D_0$. We assume that the statistician may use any, potentially randomized, algorithm $A$ which is
a measurable function of the $m$ samples and outputs the Boolean decision {YES,NO} corresponding to their prediction of whether D or D0 respectively generated the observed samples. Now, for any Boolean-valued algorithm A examining the samples, we define the advantage of $A$ solving the decision problem, as the sequence of positive numbers.
\begin{equation}
    |P_{x\in D} [\calA(x) = \text{Yes}] - P_{x\in D_0} [\calA(x) = \text{No}] |
\end{equation}

\subsubsection{Decision and Phaseless CLWE}
\begin{defi}{\textbf{Phaseless CLWE $A_{w, \beta, \gamma}$}}
We define the Phaseless-CLWE distribution on dimension d with frequency $\gamma$, $\beta-$ bounded adversarial noise, hidden direction $w$ to be the distribution of the pair $(x,z) \in \mathbb{R}^d \times [0, 1/2]$ where $x \in N(0, I_d)$ and
\begin{equation}
    z = \epsilon \gamma <w,x> + \xi \quad \text{mod} 1
\end{equation}
for some $\epsilon \in \{-1, 1\}$ such that $z \geq 0 $ and bounded noise $|\xi|< \beta$.
\end{defi}

\begin{defi}{\textbf{Decision phaseless CLWE}}. For parameters $\beta, \gamma >0 $, the average-case decision problem $\text{CLWE}_{\beta, \gamma}$ is to distinguish from i.i.d samples the following two distributions over $\mathbb{R}^d \times [0,1]$ with non-negligible advantage: 1) the Phaseless CLWE distribution $A_{w, \beta, \gamma}$ 2) $N(0, I_d) \times U[0,1]$.
\end{defi}




% \subsection{Security Analysis}
\begin{lem}  \label{lem:lemma1}
Assume $\beta \in[0, 1]$. Suppose that one receives a sample $(x, \Tilde{z})$ from the periodic neurons on dimension d with frequency $\gamma$ under $\beta$-bounded adversarial noise, and invertible periodic function $\phi: [-C, C] \to [-1, 1]$ in one single period. Let $\Bar{z} := sgn(\Tilde{z})min(1, |\Tilde{z}|)$.
Then, the pair $(x, \phi^{-1}(\Bar{z})/(2C) mod 1)$ is a sample from the Phaseless-CLWE distribution on dimension d with frequency $\gamma$ under $\frac{1}{2C}\phi^{-1}(1-\beta)$-bounded adversarial noise.
\end{lem}
According to Lemma \ref{lem:lemma1}, we could define the decision periodic neurons problem as follows:
\begin{defi}{\textbf{Decision periodic neurons}}. For parameters $\beta, \gamma >0 $, the average-case decision problem $\text{PN}_{\beta, \gamma}$ is to distinguish from i.i.d samples the following two distributions over $\mathbb{R}^d \times [0,1]$ with non-negligible advantage: 1) the Phaseless CLWE distribution $B_{w, \beta, \gamma}$ 2) $N(0, I_d) \times g(U[0,1])$, where $g: x \to \phi^{-1}(x) mod 1$.
\end{defi}

\begin{thm}
If $\phi^{-1}$ satisfies lipticiz condition, then a polynomial-time algorithm that solves \textbf{Decision phaseless CLWE} implies a polynomial-time quantum
algorithm for solving  \textbf{Decision periodic neurons}
\end{thm}

==> Section/backup.tex <==
\section{Security Analysis}


\subsection{Privacy-Preserving Capability of FedAdOb}
\label{sec:analysis}
We investigate the privacy-preserving capability of FedPass against feature reconstruction attack and label inference attack. 
% Argument for security consists of three halves: (1) To recover significant information about $x$ from the forward embedding, computationally limited eavesdroppers/attackers break AOF is difficult  (Sect. \ref{}). (2) For the passive party, ...  (Sect. \ref{}); 3) It is hard for the adversary to infer the private passport.\\
% \textbf{Attack scenario:} In each epoch, the active party observe the forward embedding of the passive party, the passive party knows backward gradients from the active party and train their passive models.
Note that we conduct the privacy analysis with linear regression models, for the sake of brevity. Proofs are deferred to Appendix D.
% Nevertheless the analysis can be applied to neural network models [citations? to support the argument]
\begin{definition} \label{def:SplitFed}
Define the forward function of the passive model $G$ and the active model $F$: 
\begin{itemize}
    \item For passive layer: $H = G(x) =  W_p s_\gamma^p \cdot W_p x + W_p s_\beta^p$.
    \item For active layer: $y = F(H) =  W_a s_\gamma^a \cdot W_a  H + W_a s_\beta^a$.
\end{itemize}
where $W_p$, $W_a$ are 2D matrices of the passive and active models; $\cdot$ denotes the inner product, $ s_\gamma^p,  s_\beta^p$ are passports of the passive party, $ s_\gamma^a,  s_\beta^a$ are passports of the active party.
% $D_\gamma$, $\hat{D_\gamma}$ are diagonal matrix of scaling weights of batch normalization or passport layer; $\mu$, $O$ are the outputs of public and private layer; $\cdot$ denotes matrix product.\\
% \textit{Remark}: Any convolution layers can be converted into a fully-connected layer by simply stacking together spatially shifted convolution kernels. (\cite{ma2017equivalence}). In addition, the scaling factor $\gamma$ of batch normalization or passport layer could be explained by a diagonal matrix in the forward function. Consequently, we use $a(D_\gamma \cdot w \cdot x + b)$ as forward function of private layer.
\end{definition}

\subsubsection{Hardness of feature Restoration with FedPass}
Consider the white-box Model Inversion (MI) attack (i.e., model inversion step in CAFE \cite{jin2021cafe,he2019model}) that aims to inverse the model $W_p$ to recover features $\hat{x}$ approximating original features $x$. In this case, the attacker (i.e., the active party) knows the passive model parameters $W_p$, forward embedding $H$ and the way of embedding passport, but does not know the passport.

\begin{theorem}\label{thm:thm1}
    Suppose the passive party protects features $x$ by inserting the $s_{\beta}^p$. The probability of recovering features by the attacker via white-box MI attack is at most $\frac{\pi^{m/2}\epsilon^m}{\Gamma(1+m/2)N^m}$ such that the recovering error is less than $\epsilon$, i.e., $\|x-\hat{x}\|_2\leq \epsilon$,
\end{theorem}
where $m$ denotes the dimension of the passport via flattening, $N$ denotes the passport range formulated in Eq. \eqref{eq:sample-pst} and $\Gamma(\cdot)$ denotes the Gamma distribution.
% \begin{proof}
%     According to Lemma \ref{lem1}, the attacker aims to recover the feature $\hat{x}$ within the $\epsilon$ error from the original feature $x$, that is, the guessed passport needs to satisfy: 
%     \begin{equation}
%         \|s_{\beta'}^p - s_\beta^p  \|_2 \leq \epsilon
%     \end{equation}
% Therefore, the area of inferred passport of attackers is sphere with the center $s_{\beta}^p$ and radius $\epsilon$. And the volumes of this area is at most $\frac{\pi^{m/2}\epsilon^m}{\Gamma(1+m/2)}$, where $F$ represent the Gamma distribution and $m$ is dimension of the passport. Consequently, the probability of attackers to successfully recover the feature within $\epsilon$ error is:
% \begin{equation*}
% \begin{split}
%         p \geq \frac{\pi^{m/2}\epsilon^m}{\Gamma(1+m/2)N^m},
%         \end{split}
% \end{equation*}
% where the whole space is $(-N,0)^m$ with volume $N^m$.
% \end{proof}
Theorem \ref{thm:thm1} demonstrates that the attacker's probability of recovering features within error $\epsilon$ is exponentially small in the dimension of passport size $m$. The successful recovering probability is inversely proportional to the passport range $N$ to the power of $m$.
% Noted that the $C$ increases as the absolute value of the passport $s_\gamma^p$ becomes large such that the recovered feature is far away from the original feature. However, the model performance is influenced when $|s_\gamma^p|$ increases (We analyze the change of privacy and model performance about $|s_\gamma^p|$ in Appendix B).
\subsubsection{Hardness of Label Recovery with FedPass}
Consider the passive model competition attack \cite{fu2022label} that aims to recover labels owned by the active party. The attacker (i.e., the passive party) leverages a small auxiliary labeled dataset $\{x_i, y_i\}_{i=1}^{n_a}$ belonging to the original training data to train the attack model $W_{att}$, and then infer labels for the test data. Note that the attacker knows the trained passive model $G$ and forward embedding $H_i = G(x_i)$. Therefore, they optimizes the attack model $W_{att}$ by minimizing $\ell = \sum_{i=1}^{n_a}\|W_{att}H_i-y_i\|_2$.
% \begin{assumption}
%     The main task algorithm of VFL on the auxiliary labeled dataset is convergent i.e., the training error goes to zero. 
% \end{assumption}
\begin{assumption}\label{assum1}
Suppose the original main algorithm of VFL is convergent. For the attack model, we assume the error of the optimized attack model $W^*_{att}$ on test data $\tilde{\ell}_t$ is larger than that of the auxiliary labeled dataset $\Tilde{\ell}_a$.
\end{assumption}
% \begin{rmk}
% The error on test data $\Tilde{\ell}_t$ is usually higher than on the auxiliary labeled dataset $\Tilde{\ell}_a$ because the former is computed on an unknown dataset that the attack model has not seen before.
% \end{rmk}
% they wants to learn a mapping from $G(x_i)=H_i$ to $y_i$, $i=1, \cdots, n$ by minimizing the regression loss $\Tilde{\ell} = \sum_{i=1}^n\|G(x_i)-y_i\|_2$. Assume the the regression loss of FedPass is zero, then $y_i = F(H_i) = W_a s_{\gamma,i}^a \cdot W_a  H_i + s_{\beta, i}^aW_a$.
\begin{theorem} \label{thm2}
Suppose the active party protect $y$ by embedding $s^a_\gamma$, and adversaries aim to recover labels on the test data with the error $\Tilde{\ell}_t$ satisfying:
    \begin{equation}
        \Tilde{\ell}_t \geq \min_{W_{att}} \sum_{i=1}^{n_a}\|(W_{att}- T_i)H_i\|_2,
    \end{equation}
    where $T_i =diag(W_as_{\gamma,i}^a) W_a$ and $s_{\gamma,i}^a$ is the passport for the label $y_i$ embedded in the active model. Moreover, if $H_{i_1} = H_{i_2} = H$ for any $1\leq i_1,i_2 \leq n_a$, then
    \begin{equation} \label{eq:protecty}
        \Tilde{\ell}_t \geq \frac{1}{(n_a-1)}\sum_{1\leq i_1<i_2\leq n_a}\|(T_{i_1}-T_{i_2})H\|_2
    \end{equation}
\end{theorem}
\begin{prop}\label{prop1}
Since passports are randomly generated and $W_a$ and $H$ are fixed, if the $W_a = I, H=\Vec{1}$, then it follows that:
\begin{equation}
    \Tilde{\ell}_t \geq \frac{1}{(n_a-1)}\sum_{1\leq i_1<i_2\leq n_a}\|s_{\gamma,i_1}^a-s_{\gamma,i_2}^a\|_2)
\end{equation}
\end{prop}
% \begin{proof}
% For only inserting the passport $s^a_\gamma$ of active party, according to Assumption \ref{assum1-app}, we have
% \begin{equation}
%     y_i=   W_a s_\gamma^a * W_a  H_i
% \end{equation}
% Moreover, the attackers aims to optimize
% \begin{equation*}
% \begin{split}
%        &\min_W\sum_{i=1}^{n_a}\|WH_i-y_i\|_2  \\
%        = &\min_W\sum_{i=1}^{n_a}\|WH_i - W_a s_\gamma^a * W_a  H_i\|_2 \\
%        =&\min_W\sum_{i=1}^{n_a}\|(W-T_i)H_i\|_2,
% \end{split}   
% \end{equation*}
% where $T_i =diag(W_as_{\gamma,i}^a) W_a$. Therefore, based on Assumption \ref{assum1-app}, $\Tilde{\ell}_t\geq \min_W\sum_{i=1}^{n_a}\|(W-T_i)H_i\|_2$. Moreover, if $H_i = H_j = H$ for any $i,j \in [n_a]$, then
% \begin{equation*}
%     \begin{split}
%         \Tilde{\ell}_t& \geq \min_W\sum_{i=1}^{n_a}\|(W-T_i)H_i\|_2 \\
%         &= \min_W \frac{1}{2(n-1)}\sum_{1\leq i,j\leq n_a}(\|(W-T_i)H\|_2+ \|(W-T_j)H\|_2) \\
%         &\geq \min_W \frac{1}{2(n-1)}\sum_{1\leq i,j\leq n_a}(\|(T_j-T_i)H\|_2) \\
%        & =  \frac{1}{(n-1)}\sum_{1\leq i<j\leq n_a}(\|(T_j-T_i)H\|_2)
%     \end{split}
% \end{equation*}
% \end{proof}

Theorem \ref{thm2} and Proposition \ref{prop1} show that the label recovery error $\Tilde{\ell}_t$ has a lower bound,
which deserves further explanations. First, when passports are randomly generated for all data, i.e., $s_{\gamma,i_1}^a \neq s_{\gamma,i_2}^a$, then a non-zero label recovery error is guaranteed no matter how adversaries attempt to minimize it. The recovery error thus acts as a protective random noise imposed on true labels. Second, the magnitude of the recovery error monotonically increases with the variance $\sigma^2$ of the Gaussian distribution passports sample from (in Eq. \eqref{eq:sample-pst}), which is a crucial parameter to control privacy-preserving capability (see Experiment results in Appendix B) are in accordance with Theorem \ref{thm2}. 
Third, it is worth noting that the lower bound is based on the training error of the auxiliary data used by adversaries to launch PMC attacks. Given possible discrepancies between the auxiliary data and private labels, e.g., in terms of distributions and the number of dataset samples, the actual recovery error of private labels can be much larger than the lower bound. Again, this strong protection is observed in experiments (see Sect. \ref{sec:exp}). 

% This lower bound deserves three explainations. First, when passports are randomly generated for all data i.e.si≠sj then a non-zero label recovery error is gurantteed no matter how adversaries attempt to to minimize it. The recovery error can be viewed as a random noise imposed on true labels.
% Second, the magnitude of the recovery error monotonically increases with the passport range  N, which is a crucial parameter to control privacy-preserving capability. Experiment results in Appendix ? are in accordance with Theorem 2. 
% Third, it is worth noting that the lower bound is based on the training error of the auxiliary data used by adversaries to launch PMC attacks. Given possible discrepancies between the auxiliary data and private labels owned by the active party, e.g. in terms of distributions and the number of dataset samples, the actual recovery error of private labels can be much larger than the lower bound. Again, this strong protection in observed in experiments (see Sect. ?). 


% which reflects the passive party cannot learn the active model $W$ well in the existence of passport. Concretely, when passports $s_{\gamma,i}^a$ embedding on \textcolor{red}{all the data} are the same,  $T_i=T_j$ (for any $i,j$) leading the lower bound to be zero. We embed different passports for different batch data (see line 13 in Algo. \ref{alg:aof-vfl}). Furthermore, when the passport range becomes large, the $\sum_{1\leq i<j\leq n_a}(\|(T_j-T_i)H\|_2)$ always increases, meaning it is hard to recover labels.
